Lattice piecewise affine approximation of explicit nonlinear model predictive control with application to trajectory tracking of mobile robot

To promote the widespread use of mobile robots in diverse fields, the performance of trajectory tracking must be ensured. To address the constraints and nonlinear features associated with mobile robot systems, we apply nonlinear model predictive control (MPC) to realize the trajectory tracking of mobile robots. Specifically, to alleviate the online computational complexity of nonlinear MPC, this paper devises a lattice piecewise affine (PWA) approximation method that can approximate both the nonlinear system and control law of explicit nonlinear MPC. The kinematic model of the mobile robot is successively linearized along the trajectory to obtain a linear time-varying description of the system, which is then expressed using a lattice PWA model. Subsequently, the nonlinear MPC problem can be transformed into a series of linear MPC problems. Furthermore, to reduce the complexity of online calculation of multiple linear MPC problems, we approximate the optimal solution of the linear MPC by using the lattice PWA model. That is, for different sampling states, the optimal control inputs are obtained, and lattice PWA approximations are constructed for the state control pairs. Simulations are performed to evaluate the performance of our method in comparison with the linear MPC and explicit linear MPC frameworks. The results show that compared with the explicit linear MPC, our method has a higher online computing speed and can decrease the offline computing time without significantly increasing the tracking error.

==> body/section5.tex <==
\subsection{Description of Overall Process}
The whole trajectory tracking process is shown in Algorithm \ref{alg:1} and Algorithm \ref{alg:2}.

%\begin{document}  		
	\begin{figure}[h]
	\centering    
%   \begin{tikzpicture}
		\scriptsize  
		\tikzstyle{format}=[rectangle,draw,thin,fill=white]  
		%定义语句块的颜色,形状和边
		\tikzstyle{test}=[diamond,aspect=2,draw,thin]  
		%定义条件块的形状,颜色
		\tikzstyle{point}=[coordinate,on grid,]  
		%像素点,用于连接转移线
		\begin{tikzpicture}%[node distance=10mm,auto,>=latex',thin,start chain=going below,every join/.style={norm},] 
		%start chain=going below指明了流程图的默认方向，node distance=8mm则指明了默认的node距离。这些可以在定义node的时候更改，比如说 
		%\node[point,right of=n3,node distance=10mm] (p0){};  
		%这里声明了node p0，它在node n3 的右边，距离是10mm。

		\node[format,text width=15.5mm] (WMR){Kinematic Model};
		\node[format,right of=WMR,text width=15.5mm,node distance=31mm] (linearize){Linearized Models};
		\node[format,right of=linearize,text width=15.5mm,node distance=38mm] (problem){Explicit Linear Problem};
		\node[format,below of=problem,text width=15.5mm,node distance=15mm] (dataset){Dataset  $\mathcal{X} \times \mathcal{U}$};
		\node[format,left of=dataset,text width=15.5mm,node distance=38mm] (lattice){Lattice PWA Approximation Model};
		\node[format,left of=lattice,text width=15.5mm,node distance=31mm] (irredundant){Simplified Lattice PWA Approximation Model};
		%\node[format] (n0) at(4,4){A}; 直接指定位置 
		%定义完node之后进行连线,
		%\draw[->] (n0.south) -- (n1); 带箭头实线
		%\draw[-] (n0.south) -- (n1); 不带箭头实线
		%\draw[<->] (n0.south) -- (n1.north);   双箭头
		%\draw[<-,dashed] (n1.south) -- (n2.north); 带箭头虚线 
		%\draw[<-] (n0.south) to node{Yes} (n1.north);  带字,字在箭头方向右边
		%\draw[->] (n1.north) to node{Yes} (n0.south);  带字,字在箭头方向左边
		%\draw[->] (n1.north) to[out=60,in=300] node{Yes} (n0.south);  曲线
		%\draw[->,draw=red](n2)--(n1);  带颜色的线
		\draw[->] (WMR)--node[above]{linearization}(linearize);
		\draw[->](linearize)--node[above]{For each different}node[below]{linearized model}(problem);
		\draw[->](problem)--node[left]{Sampling}(dataset);
		\draw[->](dataset)--(lattice);
		\draw[->](lattice)--node[above]{de-redundant}(irredundant);
		\end{tikzpicture}  
	\end{figure}  
%\end{document}  


%\begin{document}  		 
	\begin{figure}[h]
	\centering  
		\scriptsize  
		\tikzstyle{format}=[rectangle,draw,thin,fill=white]  
		%定义语句块的颜色,形状和边
		\tikzstyle{test}=[diamond,aspect=2,draw,thin]  
		%定义条件块的形状,颜色
		\tikzstyle{point}=[coordinate,on grid,]  
		%像素点,用于连接转移线
		\begin{tikzpicture}%[node distance=10mm,auto,>=latex',thin,start chain=going below,every join/.style={norm},] 
		%start chain=going below指明了流程图的默认方向，node distance=8mm则指明了默认的node距离。这些可以在定义node的时候更改，比如说 
		%\node[point,right of=n3,node distance=10mm] (p0){};  
		%这里声明了node p0，它在node n3 的右边，距离是10mm。
     \node[point](point1){};
     \node[point,right of=point1,node distance=10mm](point2){};
     \node[point,below of=point2,node distance=10mm](point6){};
		\node[format,right of=point2,text width=15mm,node distance=18mm] (model){Simplified Lattice Model};
		\node[format,right of=model,text width=12mm,node distance=27mm] (WMR){Kinematic Model};
     \node[point,right of=WMR,node distance=18mm](point3){};
     \node[point,below of=point3,node distance=10mm](point5){};
     \node[point,right of=point3,node distance=7mm](point4){};


		\draw[-] (point1)--(point2);
		\draw[->] (point2)--node[above]{$\boldsymbol{x}_{k}$}(model);
		\draw[->] (model)--node[above]{$\boldsymbol{u}_{k}$}(WMR);
		\draw[-](WMR)--node[above]{$\boldsymbol{x}_{k+1}$}(point3);
		\draw[->] (point3)--(point4);
		\draw[-] (point3)--(point5);
		\draw[-](point5)--(point6);
		\draw[->] (point6)--(point2);
		\end{tikzpicture}  
	\end{figure}  
%\end{document}  




Then we take the first reference trajectory point as the linearization point and set the linearization error to $\delta$. The first-order Taylor expansion is adopted for Equation (\ref{kinematic}) at the first reference trajectory point, and the higher-order terms are ignored to obtain
\begin{equation}
\begin{array}{ll}
\dot{\boldsymbol{x}}\!\!\!\!&=\left.\frac{\partial f\!(\boldsymbol{x}, \boldsymbol{u})}{\partial \boldsymbol{x}}\right|_{\boldsymbol{x}\!=\!\boldsymbol{x}_{r}, \boldsymbol{u}\!=\!\boldsymbol{u}_{r}}\!\cdot\! \boldsymbol{x}\!+\!\left.\frac{\partial f\!(\boldsymbol{x}, \boldsymbol{u})}{\partial \boldsymbol{u}}\right|_{\boldsymbol{x}\!=\!\boldsymbol{x}_{r}, \boldsymbol{u}\!=\!\boldsymbol{u}_{r}}\!\cdot\! \boldsymbol{u}\!+\!f\!\!\left(\boldsymbol{x}_{r}, \boldsymbol{u}_{r}\right)\\
&-\left.\frac{\partial f(\boldsymbol{x}, \boldsymbol{u})}{\partial \boldsymbol{x}}\right|_{\boldsymbol{x}=\boldsymbol{x}_{r}, \boldsymbol{u}=\boldsymbol{u}_{r}}\cdot \boldsymbol{x}_{r}\!-\!\left.\frac{\partial f(\boldsymbol{x}, \boldsymbol{u})}{\partial \boldsymbol{u}}\right|_{\boldsymbol{x}=\boldsymbol{x}_{r}, \boldsymbol{u}=\boldsymbol{u}_{r}}\cdot \boldsymbol{u}_{r}\!\\
\label{taylor}
\end{array}
\end{equation}
in which the last three terms are only related to the state and control input of the reference trajectory, so they can be regarded as a constant term. After discretization through first-order forward difference, Equation (\ref{taylor}) can be abbreviated as
\begin{equation}
\begin{array}{ll}
\boldsymbol{x}(k+1)=A(k) \boldsymbol{x}(k)+B(k) \boldsymbol{u}(k)+b(k) \\
\label{linearization}
\end{array}
\end{equation}

We number this linearization model $L_{1}$. Then the function value corresponding to the subsequent reference trajectory point is calculated successively, and the linearization error is obtained according to Equation (\ref{error}). 
\begin{equation}
\begin{array}{ll}
F_{s}=\sum_{i=1}^{n}|f(\boldsymbol{x}(k+i))-f(\boldsymbol{x}(k))|
\label{error}
\end{array}                                                                                              
\end{equation}
in which $\boldsymbol{x}(k)$ is the previous linearization point, $\boldsymbol{x}(k+n)$ represents the current reference trajectory point and $\boldsymbol{x}(k+i)$ represents the reference trajectory point between $\boldsymbol{x}(k)$ and $\boldsymbol{x}(k+n)$. When $F_{s} \geq \delta$, the previous reference trajectory point is taken as the second linearization point and the linearization model $L_{2}$ is obtained according to the above method; otherwise, the model corresponding to this point is equal to the first one and denoted as $L_{1}$, and the next reference trajectory point is continued to be considered, and so on. This method is called equivalent linearization point selection method, which ensures that the linearization error of adjacent linearization points does not exceed $\delta$.




\begin{rem}\label{Remark3}
In this paper, we use the sequential search method for the online evaluation of the explicit linear MPC algorithm, which is simple but time-consuming. And the current solution algorithm for quadratic programming is relatively mature, which makes the online calculation time of the MPC method shorter than that of explicit linear MPC.
\end{rem}
